Must the Communication Graph of MPC Protocols be an Expander?

Secure multiparty computation (MPC) on incomplete communication networks has been studied within two primary models: (1) Where a partial network is fixed a priori, and thus corruptions can occur dependent on its structure, and (2) Where edges in the communication graph are determined dynamically as part of the protocol. Whereas a rich literature has succeeded in mapping out the feasibility and limitations of graph structures supporting secure computation in the fixed-graph model (including strong classical lower bounds), these bounds do not apply in the latter dynamic-graph setting, which has recently seen exciting new results, but remains relatively unexplored. In this work, we initiate a similar foundational study of MPC within the dynamic-graph model. As a first step, we investigate the property of graph expansion. All existing protocols (implicitly or explicitly) yield communication graphs which are expanders, but it is not clear whether this is inherent. Our results consist of two types (for constant fraction of corruptions): * Upper bounds: We demonstrate secure protocols whose induced communication graphs are not expander graphs, within a wide range of settings (computational, information theoretic, with low locality, even with low locality and adaptive security), each assuming some form of input-independent setup. * Lower bounds: In the plain model (no setup) with adaptive corruptions, we demonstrate that for certain functionalities, no protocol can maintain a non-expanding communication graph against all adversarial strategies. Our lower bound relies only on protocol correctness (not privacy), and requires a surprisingly delicate argument. More generally, we provide a formal framework for analyzing the evolving communication graph of MPC protocols, giving a starting point for studying the relation between secure computation and further, more general graph properties.

==> func_comm_tree.tex <==

\begin{nfbox}{The Communication-Tree functionality}{fig:fcommtree}
\begin{center}
    \textbf{The functionality} $\fcommtree$
\end{center}
The $m$-party functionality $\fcommtree$ is parametrized by $ t\in \N $ and proceeds as follows.
\begin{enumerate}
    \item
    Every party $\Party_i$ has an empty input $ \emptystr $.
    \item
    Upon receiving a list of corrupted parties $ B\subseteq [m] $ of size $ t $ from the adversary. The functionality produces a communication tree $ \Tree $ for $ m $ parties with the following additional property:
    All but a $ 3/\log m$ fraction of the leaf nodes have a good path up to the root node (\ie a path on which majority of parties in each committee are not contained in $ B $).
    \item 
    Select input committees $ \committee_1^{\text{in}}, \ldots ,\committee_m^{\text{in}}$
    \item
    Output the description of $ \Tree $ and the input committees $ \committee_1^{\text{in}}, \ldots ,\committee_m^{\text{in}}$ to every $\Party_{i}$.
\end{enumerate}
\end{nfbox}


==> func_recon_compute_IT.tex <==

\begin{nfbox}{The IT-Reconstruct-and-Compute functionality}{fig:freconcomputeIT}
\begin{center}
    \textbf{The functionality} $\freconcomputeIT$
\end{center}
The $m$-party functionality $\freconcomputeIT$ is parametrized by $ n\in \N $ and a $(t',n')$ ECSS scheme $(\Share,\Recon)$ and proceeds as follows.
\begin{enumerate}
    \item
    Every party $\Party_i$ sends as input a list of pairs of the form $ (j,s_i^{j})$ for $ j \in \N $ and $s_i^{j} $ a share under the ECSS scheme.
    \item
    For every $j\in[n]$, let $s_1^j,\ldots,s_{n'}^j$ be all the received shares paired with the value $ j $. (If one of the parties provided invalid input, set the corresponding share to be the default value, \eg a share of zero.)
    Reconstruct $x_j=\Recon(s_1^j,\ldots,s_{n'}^j)$.
    \item
    Compute $y=f(x_1\ldots, x_n)$.
    \item
    Output $y$ to every $\Party_{i}$.
\end{enumerate}
\end{nfbox}

